The Ramshaw-Mesina Hybrid Algorithm applied to the Navier Stokes Equations

In 1991, Ramshaw and Mesina proposed a novel synthesis of penalty methods and artificial compression methods. When the two were balanced they found the combination was 3-4 orders more accurate than either alone. This report begins the study of their interesting method applied to the Navier-Stokes equations. We perform stability analysis, semi-discrete error analysis, and tests of the algorithm. Although most of the results for implicit time discretizations of our numerical tests comply with theirs for explicit time discretizations, the behavior in damping pressure oscillations and violations of incompressibility are different from their findings and our heuristic analysis.

==> introduction_old.tex <==
\section{Introduction}
The motion of a viscous, incompressible fluid is modeled by the well-known Navier-Stokes equations which consists of conservation of momentum and mass equations. Consider a regular and bounded flow domain $\Omega\subset  \mathbb{R}^d \ (d=2,\ 3)$. The Navier-Stokes equations (NSE) with no-slip boundary conditions are given as:
%\begin{equation}\label{nse}
\begin{align*}
& u_t+ u\cdot\grad u-\nu\Delta u+\grad p=f(x),\ \text{and} \ \div u=0,\ \text{in}\ \Omega\cross [0,T],
\\& u=0,\ \text{on}\ \partial \Omega \cross[0,T],\ \text{and}\ u(x,0)=u_0,\ \text{in}\ \Omega.
\end{align*}
%\end{equation}
Here $u$ is the velocity, $\nu$ is the kinematic viscosity, $p$ is the pressure, and $f$ is the prescribed body force. One of the major challenges for solving the NSE numerically is the coupling of velocity and pressure which decelerates the execution times of codes and raises the computational memory needs. Pressure penalty methods (PP) and artificial compression (AC) methods are known to perform well in terms of eliminating this coupling \cite{guzel22}.\\
In 1991, Ramshaw and Mesina proposed and tested a numerical regularization for approximating solutions of the incompressible Navier-Stokes equations by combining PP and AC methods in a novel way \cite{ramshaw1991hybrid}. Formerly, Kobelkov \cite{kobel2002symmetric} and Brooks and Hughes (in a short remark in a long paper) \cite{brooks1982streamline} have tried syntheses of penalty and artificial compression models without significant gain. 
The idea of Ramshaw and Mesina is to convert the penalty relaxation of incompressibility from $2\beta\div u+p=0$ to $\frac{d}{dt}(2\beta \div u+p)=0$ before combining with the  artificial compression relaxation $p_t+\alpha^2\div u=0$. This gives rise to a hybrid model which is then discretized in space and time. Their continuum model is to select large parameters $\alpha^{2}$\ and $\beta$ and to solve
\begin{equation}\label{nse}
\begin{aligned}
& u_t+ u\cdot\grad u+\frac{1}{2}(\div u)u-\nu\Delta u+\grad p=f(x),\ \text{in}\ \Omega\cross [0,T],
\\& p_t+\alpha^2\div u+2\beta \div u_t=0,\ \text{in}\ \Omega\cross [0,T],
\\& u=0,\ \text{on}\ \partial \Omega \cross[0,T],\ \text{and}\ u(x,0)=u_0,\ \text{in}\ \Omega.
\end{aligned}
\end{equation}
This model is a clever combination of the penalty method (replacing
$\div u=0$\ with $\div u+(2\beta)^{-1}p=0$) and the artificial compression method (replacing $\div u=0$  with  $\alpha^{-2}p_{t}+\div u=0$). Their motivating intuition was that the penalty method damps rapidly high frequency components of incompressibility violations while artificial compression method reduces those violations by moving them to higher frequencies as non-physical acoustics. To summarize, this hybrid algorithm to the Navier-Stokes equations replaces $\div u=0$ by $p_t+\alpha^2\div u+2\beta \div u_t=0$ where the coefficients $\alpha$ and $\beta$ are both supposed to be large \cite{ramshaw1991hybrid}. This decouples the velocity and pressure, making the resulting system significantly more straightforward to solve. They considered finite difference method for discretization in space and time. The numerical results of Ramshaw and Mesina have shown that, their method is more accurate compared to penalty and artificial compression methods in terms of computational time and yields divergence errors,
\begin{center}
... \emph{3-4 orders of magnitude smaller}..., \cite[page 170, point 3]{ramshaw1991hybrid}.
\end{center}
In this study, we investigate the hybrid scheme of Ramshaw and Mesina in terms of finite element spatial discretization and try to investigate the performance of the hybrid method with complete numerical analysis and computational testing. We added $\frac{1}{2}(\div u)u$ to the bilinear term to get a modified bilinear term introduced in \cite{temam}. To the best of our knowledge, this is the first study concerning the hybrid scheme of Ramshaw and Mesina in terms of the finite element method. We also consider the damping effect of the hybrid scheme and test and compare its performance with PP and AC methods. To get an idea of what to expect, we derive the associated acoustic equations for the model. This is based on assuming that $u(x,t)$ is small while the pressure is not. Thus, we start by taking the divergence of momentum equation and first-order time derivative of continuity equation in \eqref{nse} and eliminating $\div{u_t}$ to get:
$$p_{tt}-2\beta \Delta p_t-\alpha^2\Delta p=-\div{f}+\div{(u\cdot\grad u+\frac{1}{2}(\div u)u)}$$
This is the Lighthill pressure wave equation and to analyze the nonphysical acoustics, we set $\div{f}=0$ and drop the quadratic term $\div{(u\cdot\grad u+\frac{1}{2}(\div u)u)}$. This setting gives us the acoustic equation:
$$p_{tt}--2\beta \Delta p_t-\alpha^2\Delta p=0 .$$  
This is over-damped (hence no oscillations) provided:
\begin{eqnarray*}
\frac{\alpha}{\beta} &<& \sqrt{\lambda} \quad \text{where}\\
\lambda &=& \text{Eigenvalue of discrete Laplacian implied by}\\
\frac{\alpha}{\beta} &<& \sqrt{\lambda_0}
\end{eqnarray*}
with $0<\lambda_0$ being the smallest eigenvalue. Thus, a selection of $\alpha^2=O(\Dt t ^{-1}),\,\,\beta=O(\Dt t ^{-1})$ which results with $\frac{\alpha}{\beta}=O(\Dt t ^{1/2}) < \sqrt{\lambda_0}$ is consistent with given analysis.\\
%+++++++++++++++++++++++++++++++++
% The main result of this paper is the complete numerical analysis and computational testing of effective algorithms for the NSEs. 
 The paper is organized as follows. The algorithm is described in \Cref{sec:3}. The stability analysis and error analysis are given in \Cref{sec:4} and \Cref{sec:5}, respectively. Numerical tests are given in \Cref{sec:6}.
%\subsection{Related Work}


